BioLeaF: A Bio-plausible Learning Framework for Training of Spiking Neural Networks

Our brain consists of biological neurons encoding information through accurate spike timing, yet both the architecture and learning rules of our brain remain largely unknown. Comparing to the recent development of backpropagation-based (BP-based) methods that are able to train spiking neural networks (SNNs) with high accuracy, biologically plausible methods are still in their infancy. In this work, we wish to answer the question of whether it is possible to attain comparable accuracy of SNNs trained by BP-based rules with bio-plausible mechanisms. We propose a new bio-plausible learning framework, consisting of two components: a new architecture, and its supporting learning rules. With two types of cells and four types of synaptic connections, the proposed local microcircuit architecture can compute and propagate error signals through local feedback connections and support training of multi-layers SNNs with a globally defined spiking error function. Under our microcircuit architecture, we employ the Spike-Timing-Dependent-Plasticity (STDP) rule operating in local compartments to update synaptic weights and achieve supervised learning in a biologically plausible manner. Finally, We interpret the proposed framework from an optimization point of view and show the equivalence between it and the BP-based rules under a special circumstance. Our experiments show that the proposed framework demonstrates learning accuracy comparable to BP-based rules and may provide new insights on how learning is orchestrated in biological systems.

==> 9_background.tex <==
\section{Background}
\label{sec:background}
\subsection{Spiking Neuron Model}
Both pyramidal cells and SOM cells are modeled by the leaky integrate-and-fire (LIF) neuron model, which is one of the most prevalent choices for describing dynamics of spiking neurons. 
% The behavior of a LIF neuron can be described by three variables: the postsynaptic current (PSC) ${a}(t)$, the neuronal membrane potential ${u}(t)$, and the output spike train ${s}(t)$.
% All cells in our SNN despite of its type share three parameters: membrane potential's  decaying time constant $\tau_m$; the time constant of the synaptic function $\tau_s$; and the firing threshold $\vartheta$.
\subsubsection{LIF Neuron Model}
The dynamics of the neuronal membrane potential $u$ of neuron $i$ in layer $l$ is described by:
\begin{equation}
    \tau_m\frac{d {u}_i^{(l)}(t)}{d t}  = -{u}_i^{(l)}(t)+ I_i^{(l)}(t)
    % \sum_{j=1}^{N^{(l-1)}}\textcolor{ForestGreen}{w_{ij}^{(l)}}{a}_j^{(l-1)}(t)
    + \eta_i^{(l)}(t),
    \label{eq:pyramidal}
\end{equation}
where $I_i^{(l)}$ is the total input of synaptic currents, and $\eta_i^{(l)}(t)$ denotes the reset function. A spiking neuron reset its membrane potential from threshold $\vartheta$ to the resting potential $v_{\rm rest}$ (we set $v_{\rm rest}=0$) each time when it fires a spike. We model $\eta_i^{(l)}(t)$ as the time convolution (*) between a reset kernel $\nu$ and the neuron's output spike train ${s}_i^{(l)}$: $\eta_i^{(l)}(t) = (\nu \ast {s}_i^{(l)}) (t)$. The reset kernel $\nu(t)=-\vartheta\delta(t)$. The amount of resetting is equal to the threshold $\vartheta$ (we set $\vartheta=1$), and $\delta(t)$ is the Dirac delta function. The neuron's output spike train is also modeled by a serious of delta functions as:${s}_i^{(l)}=\sum_f\delta(t-t_{i(f)}^{(l)})$. Here, $t_{i(f)}^{(l)}$ represent the firing time of the $f^{th}$ spike of neuron $i$ in layer $(l)$. An output spike is generated once the membrane potential reaches the threshold $\vartheta$. Following (\# cite), we define such a spike function as:
\begin{equation}
\begin{aligned}
&f_s(u):u\rightarrow s, s(t):=s(t)+\delta(t-t_{(f+1)}),
     t_{(f+1)}={\rm min}\left\{ t: u(t)=\vartheta, t>t_{(f)}\right \}.
\end{aligned}
\end{equation}

% \subsubsection{SOM Cell}
% The role of the SOM cells are to \emph{predict} the pyramidal cells' behavior, so we add footnotes $p$ to mark all variables of SOM cells. The dynamics of SOM cells are then described by:
% \begin{equation}
%     \tau_m\frac{d {u}_{i_p}^{(l)}(t)}{d t}  = -{u}_{i_p}^{(l)}(t)+  I_{i_p}^{(l)}(t)
%     % \sum_{j=1}^{N^{(l-1)}}\textcolor{Orange}{w_{i_pj}^{(l)}}{a}_j^{(l-1)}(t) 
%     + \eta_{i_p}^{(l)}(t),
%     \label{eq:SOM}
% \end{equation}
% % where $\textcolor{Orange}{w_{i_pj}^{(l)}}$ is the synaptic connection weight between the pyramidal cell $j$ in layer $(l-1)$ and the SOM cell $i$ in layer $(l)$. 
% The reset function follows the same rule as: $\eta_{i_p}^{(l)}(t) = (\nu \ast {s}_{i_p}^{(l)})(t)$. The differences between SOM cells and pyramidal cells will be discussed in the following sections.

\subsection{Synaptic Currents}
\label{sec:synapse}
% \subsubsection{Basal Dendrites}
We model the general total input current on neuron i as:
\begin{equation}
    I_i(t) = \sum_{j}{w_{ij}}\sum_f\alpha_{ij}(t-t_{j(f)}).
\end{equation}
The modeled total input is the weighted sum over all current pulses:
\begin{equation}
    \alpha_{ij}\left(t-t_{j(f)}\right) = g_{ij}\left(t-t_{j(f)}\right)\cdot \left[E_{\rm syn}-u_i(t)\right],
\end{equation}
where $E_{\rm syn}$ is the reversal potential for the synaptic current. 
We set $E_{\rm syn}\gg\vartheta$ in all types of synapses, so the membrane potential dependency can be neglected, and the term $[E_{\rm syn}-u_i(t)]$ can be treated as a constant and absorbed into weights. 
$g_{ij}(t-t_{j(f)})$ is the synaptic conductance change. We modeled it following (\#cite), but simplified the double exponential function to a single exponential decaying function and have:
\begin{equation}
    g_{ij}\left(t-t_{j(f)}\right)=B_i(t)\cdot ({1}/{\tau_s})\cdot exp\left[-\left(t-t_{j(f)}\right)/{\tau_s}\right],
\end{equation}
where $B_i(t)$ is a membrane potential dependent gating function.  The synapses in different location have different properties, where the two types of synapse we use in this work are the \emph{forward-related-type (F-type)} and the \emph{error-related-type (E-type)}. We introduce them one by one as following:

\textbf{F-Type Synapses}:
% Input currents of Pyramidal Cells' Basal Dendrites \& Input currents of SOM Cells}:
% For these synapses on the forward pass, we set $E_{\rm syn}\gg\vartheta$ so the membrane potential dependency in the term $[E_{\rm syn}-u_i^{(l)}(t)]$ can be neglected. This term can then be treated as a constant and absorbed into weights. Further, 
$B_i(t)$ is set to 1 (voltage independent conductance) as a general setting for AMPA-based conductance. We follow this setting and the input current is then simplified to a widely-used alpha function with time constant $\tau_s$:
\begin{equation}
    \alpha_{ij}\left(t-t_{j(f)}\right) = ({1}/{\tau_s})\cdot exp\left[-\left(t-t_{j(f)}\right)/{\tau_s}\right].
    \label{eq:Ftype1}
\end{equation}
Under such setting, the synaptic current is independent from neuron $i$, and all postsynaptic current (PSC) generated from neuron $j$ can be uniformly expressed by one variable $a_j$ as:
\begin{equation}
    a_j(t)=\sum_f\alpha_{ij}(t-t_{j(f)})=(s_j*\epsilon)(t),~~~~\epsilon(t) = ({1}/{\tau_s})\cdot exp{(-t/{\tau_s})} H(t),
    \label{eq:Ftype2}
\end{equation}
where (*) represents the time convolution. $\epsilon(\cdot)$ is the impulse response. $H(\cdot)$ represents the Heaviside
step function: $H(t)=1, t\geq 0$ and  $H(t)=0, t<0$.

\textbf{E-Type Synapses}:
% Input Currents of Pyramidal Cells' Apical Dendrites \& Error Inputs of SOM Cells}:
$B_i(t)$ was set to be voltage dependent here, like how prior works model the NMDA-based synapses. We define $B_i(t)$ of our synapses on the apical dendrites as following:
\begin{equation}
    B_i(t) = \frac{g_{\rm max}}{1+exp\left[-k \left(u_i(t)-u_0\right)\right]\cdot[{\rm Mg^{2+}}]\cdot n},
\end{equation}
where the extracellular magnesium concentration $[{\rm Mg^{2+}}]$ was 1 mM in the model. We shift the voltage dependency of $B_i(t)$ by $u_0$, and tune the parameters $g_{\rm max}$, $k$ and $n$ to fits the function $B$ into our simplified setting where $v_{\rm rest}=0$, and $\vartheta=1$.

% Two types of synapses are used here: The top-down feedback currents from the pyramidal cell $j$ in layer $(l)$ are modeled using the excitatory NMDA-based synaptic currents model, and the 


\subsection{Bio-plausible Learning Rules}
The two bio-plausible learning rules to be discussed here are the STDP rule and the WH rule.
\subsubsection{Spike-Timing-Dependent-Plasticity (STDP)}


% Moreover, the STDP rule also includes an asymmetric non‑causal part: A synaptic connection will be weakened if its presynaptic neuron fires right after the firing of the postsynaptic neuron. 

We first introduce a popular version of the STDP rules: $\Delta w_{ij}=\sum_m\sum_n \kappa_{\rm STDP}(t_{i}^{m}-t_{j}^{n})$, where $\kappa_{\rm STDP}$ is the STDP kernel function, which is modeled by the two-sides exponential decaying function defined as:
\begin{equation}
    \kappa_{\rm STDP}(\Delta t) = \left\{
    \begin{array}{lr}
    A^+ \cdot exp(-{\Delta t}/{\tau_+}),& \Delta t>0 \\
     -A^- \cdot exp({\Delta t}/{\tau_-}),& \Delta t<0
    \end{array}\right.
    \label{eq:STDPkernel}
\end{equation}
Meantime, we define a reversed STDP kernel function $\tilde{\kappa}_{\rm STDP}(t) = \kappa_{\rm STDP}(-t)$. Recalling that all spike trains are a serious of delta function ${s}=\sum_f\delta(t-t_{(f)})$, and considering the delta function's sampling property $\int [f(t) \delta(t-T)]~dt=f(T)$, we rewrite the STDP updating rule into two equivalent forms:
\begin{equation}
% \begin{aligned}
    \Delta w_{ij}=\eta_{ij}\int (s_j \ast \kappa_{\rm STDP})(t) \cdot s_i(t)~dt
                =\eta_{ij}\int s_j(t) \cdot (s_i\ast \tilde{\kappa}_{\rm STDP})(t)~dt,
% \end{aligned}
\label{eq:int_STDP}
\end{equation}
where $\eta_{ij}$ is the learning rate. Although $\eta_{ij}$ can be absorbed into $A^+$ and $A^-$, we explicitly define it for clarity.

\subsubsection{Widrow-Hoff (WH) Learning rule}
Since the WH rule can be interpreted as an STDP-like process between the presynaptic spike trains $s_j$ and an error signal $e_i:=s_i^{\rm teach}-s_i$. In this work, we represent both the STDP rule and the WH rule uniformly as ${\rm STDP}(\cdot,\cdot)$, where the STDP rule is: ${\rm STDP}(s_{pre},s_{post})$, and the WH rule is: ${\rm STDP}(s_{pre},e_{post})$. In addition,  WH rule's kernel function $\kappa_{\rm WH}$ is usually equal to $\kappa_{\rm STDP}$ as in (\ref{eq:STDPkernel}). Defining the reverse kernel function $\tilde{\kappa}_{\rm WH}(t) = \kappa_{\rm WH}(-t)$, we have the weight updating rule of the WH rule as:
\begin{equation}
% \begin{aligned}
    \Delta w_{ij}=\eta_{ij}\int (s_j \ast \kappa_{\rm WH})(t) \cdot e_i(t)~dt
                =\eta_{ij}\int s_j(t) \cdot (e_i \ast \tilde{\kappa}_{\rm WH})(t)~dt.
% \end{aligned}
\label{eq:int_WH}
\end{equation}
It is noteworthy that the WH-based rules provides a fixed point in the weight space, $\Delta w_{ij}=0$ when $e_i=0$, which means $s_i^{\rm teach}=s_i$. It is a global positive attractor under certain conditions (\# cite).


==> 9_methods.tex <==
\section{Methods}
\subsection{Microcircuit Architecture}
\label{sec:microcircuit}
When introducing our microcircuit architecture, all connections are classified by their synaptic types as in section \ref{sec:synapse}, and only the connection rule of fully connected layers is provided, for other layers like convolution layers can be easily converted to fully connected layers.

\textbf{F-Type Synapses}:
The connections from the outputs of pyramidal cells in one layer to the basal dendrites of pyramidal cells in their next layer carrying important feature information build up the main architecture in a spiking neural networks. When training is finished, only these forward connections are needed to realize inference. The F-type synapses model defined in (\ref{eq:Ftype1}) and (\ref{eq:Ftype2}) is applied here, so the connectivity can be described through the current flows as:
\begin{equation}
    I_i^{(l)}(t) = \sum_{j=1}^{N^{(l-1)}}\textcolor{ForestGreen}{w_{ij}^{(l)}}\sum_f\alpha_{ij}(t-t_{j(f)}^{(l-1)}) = \sum_{j=1}^{N^{(l-1)}}\textcolor{ForestGreen}{w_{ij}^{(l)}}a_j^{(l-1)}(t).
\end{equation}
Referring to Figure \ref{fig:framework} (c), where the forward weights are green colored solid arrows, the weights $\textcolor{ForestGreen}{w_{ij}^{(l)}}$ are also colored green here for reader's convenience.

We then introduce the F-type predict connections as shown in orange colored solid arrows in Figure \ref{fig:framework} (c) through modeling the total current of the SOM cells $I_{i_p}^{(l)}$ as:
\begin{equation}
    I_{i_p}^{(l)}(t) = \sum_{j=1}^{N^{(l-1)}}\textcolor{Orange}{w_{i_pj}^{(l)}}\sum_f\alpha_{i_pj}(t-t_{j(f)}^{(l-1)})=\sum_{j=1}^{N^{(l-1)}}\textcolor{Orange}{w_{i_pj}^{(l)}}a_j^{(l-1)},
\end{equation}
where the footnote $p$ represent the predict-related, or the SOM-related variables.

\textbf{E-Type Synapses}:
In our predictive coding framework, the SOM cells should mimic the behavior of the same layer's pyramidal cells one-on-one. Therefore, a one-to-one teaching current from a pyramidal cell to its corresponding SOM cell (dashed purple arrows in Figure \ref{fig:framework} (c)) are needed. Together with the negative feedback output currents that SOM cells generated themselves, we get the local error signals $e_{i_p}^{(l)}$ of an SOM cell $i$ in layer $(l)$:
\begin{equation}
    e_{i_p}^{(l)}(t) = \alpha_{i_pj}^{(l)}(t)-\alpha_{i_pi_p}^{(l)}(t) =B_{i_p}^{(l)}(t) \left[a_i^{(l)}(t)-a_{i_p}^{(l)}(t)\right].
    \label{eq:SOM_error}
\end{equation}
Although this simplified one-to-one setting impose special constrains on the neural network's connectivity, the recent monosynaptic experiments confirm that the SOM cells do receive top-down connections which may encode such teaching information (\# cite). 

In the framework of predictive coding, local error signals are defined by the difference between the local layer's prediction and the real output activity from relatively higher levels in a cortical hierarchy. The real status of higher levels pyramidal neuron is its PSC coupled by the top-down error signal. We model this coupling effect by the current sum of both a neuron's PSC $a_i^{(l)}(t)$ and its error signal $e_i^{(l)}(t)$. As in Figure \ref{fig:framework} (c), we define the error signals on the pyramidal cells' apical dendrites as:
\begin{equation}
    e_j^{(l-1)}(t)=B_{j}^{(l-1)}(t)\left[\sum_{i=1}^{N^{(l)}}\left(\textcolor{Red}{w_{ji_e}^{(l)}}(a_i^{(l)}(t)+e_i^{(l)}(t))-\textcolor{NavyBlue}{w_{ji_{pe}}^{(l)}}a_{i_p}^{(l)}(t)\right)\right],
    \label{eq:pyramidal_error}
\end{equation}
where $\textcolor{Red}{w_{ij_e}^{(l)}}$ is the top-down feedback signal from the pyramidal neuron $j$ in layer $(l)$ to the apical dendrite of the pyramidal neuron $i$ in layer $(l-1)$, and $\textcolor{NavyBlue}{w_{ji_{pe}}^{(l)}}$ with both footnotes $p$ and $e$ stands for the connection weights of current from SOM cell to the apical dendrites of pyramidal cells, where the error information is encoded. For the output layer, the apical dendrites of the output pyramidal cells receives the one-on-one error signal from higher brain areas:
\begin{equation}
    e_i^{(l_N)}(t) = B_{i}^{(l_N)}(t)\left[a_i^{\rm target}(t) - a_i^{(l_N)}(t)\right]
    \label{eq:bio-error}
\end{equation}

The SOM cells differs from the pyramidal cells by the sign of their output currents, but it does not mean that we fix the type of a cell to be excitatory or inhibitory. Instead, we allow the synapses' connection weights to move across zero freely and change the sign of its current, which is a general setting in previous works (\#cite). When currents from both SOM cells and pyramidal cells summed together into the SOM cells or the apical dendrites as in (\ref{eq:SOM_error}) and (\ref{eq:pyramidal_error}), a minus sign is added for SOM cell's outputs.

\subsection{Synaptic Learning Rules}
We first conclude our synaptic learning rules as following:
\begin{equation}
% \begin{aligned}
    \Delta \textcolor{ForestGreen}{w_{ij}^{(l)}} = {\rm STDP}(s_j^{(l-1)}, e_i^{(l)})
    =\eta_{ij}\int\left( s_j^{(l-1)}(t)\ast  \kappa_{\rm STDP}\right) (t)\cdot e_i^{(l)}(t) dt
% \end{aligned}
\label{eq:forward_weights}
\end{equation}
\begin{equation}
% \begin{aligned}
    \Delta \textcolor{Orange}{w_{i_pj}^{(l)}} = {\rm STDP}(s_j^{(l-1)}, e_{i_p}^{(l)})
    =\eta_{i_pj}\int \left(s_j^{(l-1)}(t)\ast  \kappa_{\rm STDP}\right)(t)\cdot e_{i_p}^{(l)}(t) dt
% \end{aligned}
\label{eq:predict_weights}
\end{equation}
\begin{equation}
% \begin{aligned}
    \Delta \textcolor{NavyBlue}{w_{ji_{pe}}^{(l)}} = {\rm STDP}(s_{i_p}^{(l)}, e_j^{(l-1)})
    =-\eta_{ji_{pe}}\int \left(s_{i_p}^{(l)}(t)\ast \kappa_{\rm STDP}\right)(t)\cdot e_j^{(l-1)}(t)dt
% \end{aligned}
\label{eq:error_weights}
\end{equation}
% \begin{equation}
% \Delta = ?
% \end{equation}
where $\eta_{ij},\eta_{i_pj}$, and $\eta_{ji_{pe}}$ are three different learning rates for these three types of synaptic connections. In the above three equations, all the adjusting rules of a synapse can be described as a STDP process between a presynaptic current and a postsynaptic error signal, which exploits great biological plausibility. The top-down synaptic weights $\textcolor{Red}{w_{ji_{e}}^{(l)}}$ are set to be equal to the bottom-up forward weights $\textcolor{ForestGreen}{w_{ij}^{(l)}}$ for simplicity. One can also try to fixed the top-down weights $\textcolor{Red}{w_{ji_{e}}^{(l)}}$ as randomly initialized values following the idea of the feedback alignment (\#cite). 

We interpret each type of synapses' learning rule as following:

In (\ref{eq:forward_weights}), $\textcolor{ForestGreen}{w_{ij}^{(l)}}$ represents the forward weights. It's fixed point $e_i^{(l)}(t)=B_{i}^{(l_N)}(t)[a_i^{\rm target}(t) - a_i^{(l_N)}(t)]=0$ forms a positive attractor to minimize the error signal. When training is converged, we expect $a_i^{(l_N)}\approx a_i^{\rm target}$ for all pyramidal cells $(i = 1,\dots, N^{(l)}), (l=1,\dots,l_N)$.

% For the output layer, the error signal $e_i^{(l_N)}(t) = B_{i}^{(l_N)}(t)\left[a_i^{\rm target}(t) - a_i^{(l_N)}(t)\right]$ also has another meaning, which implies the loss function we used is the Van Rossum distance (\#cite) between a target spike train $s_i^{\rm target}(t)$ and the output spike train $s_i^{(l_N)}$. We denote the loss function by $L = \sum_{i=1}^{N^{(l_N)}}\int E_i(t) dt$, where $N^{(l_N)}$ is the number of pyramidal cells in the output layer $l_N$, and $E_i(t)$ is the loss of the pyramidal cell $i$ at $t$. Specifically, $L$ is given by:
% % \vspace{-0.4cm}
% \begin{equation}
% % \begin{aligned}
%     L = \sum_{i=1}^{N^{(l_N)}} \int \frac{1}{2}\left((\epsilon\ast s_i^{\rm target})(t)-(\epsilon\ast s_i^{(l_N)})(t)\right)^2
%     =\sum_{i=1}^{N^{(l_N)}} \int \frac{1}{2}\left(a_i^{\rm target}(t) - a_i^{(l_N)}(t)\right)^2
%     \label{eq:Loss}
% % \end{aligned}
% \end{equation}
% from which we can get the derivative of $L$ with respect to an output neuron's PSC $a_i^{(l_N)}$ at $t$ equal to our defined error signal $e_i^{(l_N)}(t)$:
% \begin{equation}
%     \frac{\partial L}{\partial a_i^{(l_N)}(t)} = \frac{\partial E_i(t)}{\partial a_i^{(l_N)}(t)} = \frac{\partial \frac{1}{2}\left(a_i^{\rm target}(t) - a_i^{(l_N)}(t)\right)^2}{\partial a_i^{(l_N)}(t)} = e_i^{(l_N)}(t)
% \end{equation}
% When training is converged, we expect the error signal $e_i^{(l)}$ of all pyramidal cells $i = 1,\dots, N^{(l)}, l=1,\dots,l_N$ are close to zero, by then $\frac{\partial L}{\partial a_i^{(l_N)}(t)}$ is also close to zero, and an stationary point of $L$ is reached. One can easily integrate other differentiable loss functions into our framework by substituting the error signal $e_i^{(l_N)}$ using the $\frac{\partial L}{\partial a_i^{(l_N)}(t)}$ calculated by their customized loss functions.

In (\ref{eq:predict_weights}), $\textcolor{Orange}{w_{i_pj}^{(l)}}$ stands for the predictive connections. Its fixed point in our learning rule is $e_{i_p}^{(l)}(t) = B_{i_p}^{(l)}(t) [a_i^{(l)}(t)-a_{i_p}^{(l)}(t)] = 0$, which means $a_i^{(l)}=a_{i_p}^{(l)}$, and $s_i^{(l)}=s_{i_p}^{(l)}$. As compared to (\ref{eq:forward_weights}), the learning rule of (\ref{eq:predict_weights}) does not have a fixed target signal, but needs to follow the continuously changing behavior of each SOM cell's corresponding pyramidal cell during training. 
% Empirically, the learning rate $\eta_{i_pj}$ of these predictive connections needs to be larger than the learning rate of the forward connections $\eta_{ij}$ to be able to follow the change of $\eta_{ij}$. 

The learning rule (\ref{eq:error_weights}) minimizes the norm of $e_j^{(l-1)}(t)$ in (\ref{eq:pyramidal_error}) through adjusting $\textcolor{NavyBlue}{w_{ji_{pe}}^{(l)}}$, which is equivalent to solving a linear equation:
\begin{equation}
    \sum_{i=1}^{N^{(l)}}\textcolor{NavyBlue}{w_{ji_{pe}}^{(l)}}a_{i_p}^{(l)}(t)=\sum_{i=1}^{N^{(l)}}\textcolor{Red}{w_{ji_e}^{(l)}}(a_i^{(l)}(t)+e_i^{(l)}(t)).
\end{equation}
Considering the Current-Time as a continuous $f(X)\leftrightarrow X$ function space, where all SOM cells' PSCs $a_{i_p}^{(l)}, (i=1,\dots N_l)$ form a basis of the space. Then the goal here is to restore the summed currents of all pyramidal cells in layer $(l)$ through these basis functions. When a predictive weight $\textcolor{Orange}{w_{i_pj}^{(l)}}$ is well adjusted, $a_i^{(l)}$ approximately equals to $a_{i_p}^{(l)}$, then an obvious solution to the equation above will be letting $\textcolor{NavyBlue}{w_{ji_{pe}}^{(l)}}$ equal to $\textcolor{Red}{w_{ji_e}^{(l)}}$, if we consider the error currents $e_i^{(l)}(t)$ as the orthogonal uncorrelated signal to the basis.

% As a conclusion, while updating the forward weights $\textcolor{ForestGreen}{w_{ij}^{(l)}}$ to minimize the error on the outputs of a spiking neural network, the synaptic learning rules wish to maintain the relationship of $\textcolor{ForestGreen}{w_{ij}^{(l)}}=\textcolor{Orange}{w_{i_pj}^{(l)}}=\textcolor{NavyBlue}{w_{ji_{pe}}^{(l)}}=\textcolor{Red}{w_{ji_e}^{(l)}}$ in all layers.

==> outdated_2_background.tex <==
\section{Background}


% The $0^{th}$ input layer consists of sensory cells, for example, they are photoreceptor cells in vision tasks. The $1^{st}$ hidden layer has three pyramidal neurons without SST cell. The $2^{nd}$ hidden layer 
% The somatic zone records a somatic membrane potential, which accumulates input currents and will be reset to the resting potential after each fire. The apical zone encodes an error signal generated locally from the mismatch between the top-down feedback and the prediction of SST cells. 



\subsection{Spiking Neuron Model}
Both of the pyramidal cells and SST cells are modeled by the leaky integrate-and-fire (LIF) neuron model. The LIF model is one of the most prevalent choices for describing dynamics of spiking neurons. The behavior of a LIF neuron can be described by three variables: the postsynaptic current (PSC) ${a}(t)$, the neuronal membrane potential ${u}(t)$, and the output spike train ${s}(t)$. All cells in our SNN despite of its type share three parameters: membrane potential's  decaying time constant $\tau_m$; the time constant of the synaptic function $\tau_s$; and the firing threshold $\vartheta$.
\subsubsection{Pyramidal Cell}
The dynamics of neuron $i$ in layer $l$ is described by:
\begin{equation}
    \tau_m\frac{d {u}_i^{(l)}(t)}{d t}  = -{u}_i^{(l)}(t)+ \sum_{j=1}^{N^{(l-1)}}\textcolor{ForestGreen}{w_{ij}^{(l)}}{a}_j^{(l-1)}(t) + \eta_i^{(l)}(t),
    \label{eq:pyramidal}
\end{equation}
where $\textcolor{ForestGreen}{w_{ij}^{(l)}}$ is the weight of the synapse between the pyramidal neuron $j$ in layer $(l-1)$ and the pyramidal neuron $i$ in layer $(l)$. $\eta_i^{(l)}(t)$ denotes the reset function. The PSC and the reset function can be written as:
\begin{equation}
    {a}_j^{(l-1)}(t) = (\epsilon \ast {s}_j^{(l-1)}) (t),~~~~~  \eta_i^{(l)}(t) = (\nu \ast {s}_i^{(l)}) (t),
    \label{eq:PSCReset}
\end{equation}
where (*) represents the time convolution. $\epsilon(\cdot)$ and $\nu(\cdot)$ are the impulse response and the reset kernel, respectively. The spike train is modeled as a serious of delta function:
\begin{equation}
    {s}_i^{(l)}=\sum_f\delta(t-t_{i}^{(l)f}).
    \label{eq:spike_train}
\end{equation} 
Here $t_{j}^{(l)f}$ represent the firing time of the $f^{th}$ spike of neuron $j$ in layer $(l)$. An output spike is generated once the membrane potential reaches the threshold $\vartheta$. Following (\# cite), we define such a spike function as:
\begin{equation}
\begin{aligned}
&f_s(u):u\rightarrow s, s(t):=s(t)+\delta(t-t_{(f+1)}),
     t_{(f+1)}={\rm min}\left\{ t: u(t)=\vartheta, t>t^{(f)}\right \}.
\end{aligned}
\end{equation}
In this work, a first order synaptic impulse response model, and a reset kernel without refractory period is applied:
\begin{equation}
    \epsilon(t) = \frac{1}{\tau_s}e^{(-t/{\tau_s})} H(t),~~~~ \nu(t) = -\vartheta\delta(t),
    \label{eq:epsilon}
\end{equation}
where $({1}/{\tau_s})$ is a normalization term, which guarantees that $(\int \epsilon(t) dt=1)$; $\vartheta$, the firing threshold, is the amount of membrane potential needs to be reset to the resting potential zero; and $H(\cdot)$ represents the Heaviside
step function: $H(t)=1, t\geq 0$ and  $H(t)=0, t<0$. Alternatively, the PSC function can be rewritten in a differential form as:$\tau_s \frac{d {a}_j^{(l)}(t)}{d t} = -{a}_j^{(l)}(t) + {s}_j^{(l)}(t)$.

\subsubsection{SST Cell}
The role of the SST cells are to \emph{predict} the pyramidal cells' behavior, so we add footnotes $p$ to mark all variables of SST cells. The dynamics of SST cells are then described by:
\begin{equation}
    \tau_m\frac{d {u}_{i_p}^{(l)}(t)}{d t}  = -{u}_{i_p}^{(l)}(t)+ \sum_{j=1}^{N^{(l-1)}}\textcolor{Orange}{w_{i_pj}^{(l)}}{a}_j^{(l-1)}(t) + \eta_{i_p}^{(l)}(t),
    \label{eq:SST}
\end{equation}
where $\textcolor{Orange}{w_{i_pj}^{(l)}}$ is the synaptic connection weight between the pyramidal cell $j$ in layer $(l-1)$ and the SST cell $i$ in layer $(l)$. The reset function follows the same rule as in (\ref{eq:PSCReset}) as: $\eta_{i_p}^{(l)}(t) = (\nu \ast {s}_{i_p}^{(l)})(t)$. The most important difference between SST cells and pyramidal cells is that: compared to (\ref{eq:PSCReset}), SST cells emit 'negative' PSCs: \begin{equation}
    {a}_{i_p}^{(l)}(t) = -(\epsilon \ast {s}_{j_p}^{(l)}) (t).
    \label{eq:negative_psc}
\end{equation}

\subsection{Bio-plausible Learning Rules}
The two bio-plausible learning rules to be discussed here are the STDP rule and the WH rule.
\subsubsection{Spike-Timing-Dependent-Plasticity (STDP)}
The STDP learning rule is built upon the Hebbian learning rule, which can be informally described as: "Cells that fire together, wire together" (\# cite). Following this rule, the STDP rule adjusts synaptic weights by evaluating the precise timing causal correlation: If a presynaptic neuron fires before a postsynaptic neuron, which means the PSC induced by the presynaptic spike contributes to the firing of the postsynaptic neuron, their connection is strengthened. Moreover, the STDP rule also includes an asymmetric non‑causal part: A synaptic connection will be weaken if its presynaptic neuron fires right after the firing of the postsynaptic neuron. 

We first introduce a popular version of STDP rules:
\begin{equation}
    \Delta w_{ij}=\sum_m\sum_n \kappa_{\rm STDP}(t_{i}^{m}-t_{j}^{n}),
    \label{eq:sum_STDP}
\end{equation}
where $\kappa_{\rm STDP}$ is the STDP kernel function, which is modeled by the two-sides exponential decaying function defined as:
\begin{equation}
    \kappa_{\rm STDP}(\Delta t) = \left\{
    \begin{array}{lr}
    A^+ e^{-\frac{\Delta t}{\tau_+}},& \Delta t>0 \\
     -A^- e^{\frac{\Delta t}{\tau_-}},& \Delta t<0
    \end{array}\right.
    \label{eq:STDPkernel}
\end{equation}
Meantime, we define a reversed STDP kernel function as $\tilde{\kappa}_{\rm STDP}(t) = \kappa_{\rm STDP}(-t)$. Considering all spike trains are a serious of delta function as defined in (\ref{eq:spike_train}), and the delta function's property $\int [f(t) \delta(t-t')]~dt=f(t')$, we rewrite (\ref{eq:sum_STDP}) into two equivalent expressions as:
\begin{equation}
% \begin{aligned}
    \Delta w_{ij}=\eta_{ij}\int (s_j \ast \kappa_{\rm STDP})(t) \cdot s_i(t)~dt
                =\eta_{ij}\int s_j(t) \cdot (s_i\ast \tilde{\kappa}_{\rm STDP})(t)~dt,
% \end{aligned}
\label{eq:int_STDP}
\end{equation}
where $\eta_{ij}$ is the learning rate. 

\subsubsection{Widrow-Hoff (WH) Learning rule}
The WH learning rule (\# cite) is originally a gradient descent rule for the least mean square problem. (\# cite) presented a spiking analogy to the classical WH rule for spiking neuron models, and their rule can be interpreted as an STDP-like process between the presynaptic spike trains $s_j$ and an error signal of the form $e_i:=s_i^{\rm teach}-s_i$. So, we can use a uniform form to represent these two rules as ${\rm STDP}(\cdot,\cdot)$, where the STDP rule is: ${\rm STDP}(s_{pre},s_{post})$, and the WH rule is: ${\rm STDP}(s_{pre},e_{post})$. In addition,  WH rule's kernel function $\kappa_{\rm WH}$ is usually equal to $\kappa_{\rm STDP}$ as in (\ref{eq:STDPkernel}). Defining $\tilde{\kappa}_{\rm WH}(t) = \kappa_{\rm WH}(-t)$, we have the weight updating rule of the WH rule as:
\begin{equation}
% \begin{aligned}
    \Delta w_{ij}=\eta_{ij}\int (s_j \ast \kappa_{\rm WH})(t) \cdot e_i(t)~dt
                =\eta_{ij}\int s_j(t) \cdot (e_i \ast \tilde{\kappa}_{\rm WH})(t)~dt.
% \end{aligned}
\label{eq:int_WH}
\end{equation}
The WH-based rules provides a fixed point in the weight space, that $\Delta w_{ij}=0$ only when $s_i^{\rm teach}=s_i$, which is a global positive attractor under certain conditions (\# cite).

==> outdated_3_methods.tex <==
\section{Methods}

\subsection{Microcircuit Architecture}
Define all input currents of neuron $i$ in layer $(l)$  weighted by the feed-forward connections as $\xi_i^{(l)}$, we have:
\begin{equation}
    {\xi}_i^{(l)}(t) = \sum_{j=1}^{N^{(l-1)}}\textcolor{ForestGreen}{w_{ij}^{(l)}}{a}_j^{(l-1)}(t).
\end{equation}
Referring to (\ref{eq:pyramidal}), we use the green colored $\textcolor{ForestGreen}{w_{ij}^{(l)}}$ to represent these feed-forward weights aligning with the color used in Figure \ref{fig:Methods} (a).
When training is finished, only these green feed-forward connections and the pyramidal cells are needed to realize inference.

We then define all input currents of the $i^{th}$ SOM cell in layer $(l)$ weighted by their corresponding weights $\textcolor{Orange}{w_{i_pj}^{(l)}}$ as $\xi_{i_p}^{(l)}$, then we have:
\begin{equation}
    {\xi}_{i_p}^{(l)}(t) = \sum_{j=1}^{N^{(l-1)}}\textcolor{Orange}{w_{i_pj}^{(l)}}{a}_j^{(l-1)}(t).
\end{equation}
The predict weights are colored orange as the same as the arrows' color in  (\ref{eq:SOM}) and Figure \ref{fig:micro_circuit} (c). In our predictive coding framework, the SOM cells should mimic the behavior of pyramidal cells in the same layer one-on-one . Therefore, a one-to-one teaching currents (purple arrows) are needed within a layer from pyramidal cells to SOM cells. Together with the negative feedback output currents that SOM cells generated themselves, we have the local error signals $e_{i_p}^{(l)}$ of an SOM cell $i$ in layer $(l)$ as:
\begin{equation}
    e_{i_p}^{(l)}(t) = a_i^{(l)}(t)+a_{i_p}^{(l)}(t).
\end{equation}
Although this simplified one-to-one setting impose special constrains on the neural network's connectivity, the recent monosynaptic experiments do confirm that the SOM cells do receive top-down connections which may encode such teaching information (\# cite). 

As in Figure \ref{fig:Methods} (a), we define the error signals on the pyramidal cells' apical dendrites as:
\begin{equation}
    e_j^{(l-1)}(t)=\sum_{i=1}^{N^{(l)}}\left[\textcolor{Red}{w_{ji_e}^{(l)}}(a_i^{(l)}(t)+e_i^{(l)}(t))+\textcolor{NavyBlue}{w_{ji_{pe}}^{(l)}}a_{i_p}^{(l)}(t)\right],
\end{equation}
where $\textcolor{Red}{w_{ij_e}^{(l)}}$ is the top-down feedback signal from the pyramidal neuron $j$ in layer $(l)$ to the apical dendrite of the pyramidal neuron $i$ in layer $(l-1)$. For the output layer, the apical dendrites of the output pyramidal cells receives the one-on-one error signal from higher brain areas:
\begin{equation}
    e_i^{(l_N)}(t) = a_i^{\rm target}(t) - a_i^{(l_N)}(t)
\end{equation}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{methods.pdf}
    \caption{(a) Highlighted connections between two pyramidal cells and a SOM cell (b) The new STDP curves after our modification}
    \label{fig:Methods}
\end{figure}

\subsection{Modified STDP}

Traditionally, the STDP rule is defined on the spikes - $s$. Here, we wish to extend it to PSCs - $(a=s*\epsilon)$ based on the fact that all the signals that transmit between spiking neurons are PSCs, which are continuous current signals instead of the pure point-process spike signals. More important, our STDP rule shares a great similarity with the BP algorithm, which will be fully discussed in the next section. Based on the two reasons above, we choose to substitute all $s$ in (\ref{eq:int_STDP}) to $a$, and get a modified version of the widely used STDP rule ${\rm STDP}(a_{pre},a_{post})$ as:
\begin{equation}
% \begin{aligned}
    \Delta w_{ij}=\eta_{ij}\int (a_j \ast \kappa_{\rm STDP})(t) \cdot a_i(t)~dt
                % &= \eta_{ij}\int  (s_j\ast\epsilon \ast \kappa_{\rm STDP})(t) \cdot (s_i\ast\epsilon)(t)~dt\\
                = \eta_{ij}\int \left[s_j\ast(\epsilon \ast \kappa_{\rm STDP} \ast\tilde{\epsilon})\right](t) \cdot s_i(t)~dt,
                % &=\eta_{ij}\int a_j(t) \cdot (a_i\ast \tilde{\kappa}_{\rm STDP})(t)~dt
% \end{aligned}
\label{eq:soft_int_STDP}
\end{equation}
where we can also interpret it as modifying the kernel function to a new one:
\begin{equation}
    \kappa(\Delta t) = \left(\epsilon \ast \kappa_{\rm STDP} \ast\tilde{\epsilon} \right)(\Delta t).
\end{equation}
We are allowed to do so when $\tau_s\ll(\tau_+~{\rm or}~\tau_-)$. As shown in Figure \ref{fig:Methods} (b), we measure how the kernel function $\kappa(\Delta t)$ would change after the substitution. We notice that: the new $\kappa(\Delta t)$ is a smoothed version of $\kappa_{\rm STDP}(\Delta t)$, the smaller the $\tau_s$, the more "sharp" of the PSC signal, which means the similar between $a$ and $s$, and therefore the similar between $\kappa(\Delta t)$ and $\kappa_{\rm STDP} (\Delta t)$.
Next, we can naturally extend it to the form of ${\rm STDP}(a_{pre},e_{post})$, where $e$ is the \emph{PSC-based} error signal as described in the above section, which also slightly differs from the traditional \emph{spike-based} WH rule. As compared to ${\rm STDP}(a_{pre},a_{post})$, substitution $a_{post}$ to $e_{post}$ will provide a negative feedback into the learning framework to realize accurate weight nudging, which we believe can better explain the synaptic connections with variety strength as observed in our brain.

\subsection{Synaptic Learning Rules}
We first conclude our synaptic learning rules as following:
\begin{equation}
% \begin{aligned}
    \Delta \textcolor{ForestGreen}{w_{ij}^{(l)}} = {\rm STDP}(a_j^{(l-1)}, e_i^{(l)})
    =\eta_{ij}\int\left( a_j^{(l-1)}(t)\ast  \kappa\right) (t)\cdot e_i^{(l)}(t) dt
% \end{aligned}
\label{eq:forward_weights}
\end{equation}
\begin{equation}
% \begin{aligned}
    \Delta \textcolor{Orange}{w_{i_pj}^{(l)}} = {\rm STDP}(a_j^{(l-1)}, e_{i_p}^{(l)})
    =\eta_{i_pj}\int \left(a_j^{(l-1)}(t)\ast  \kappa\right)(t)\cdot e_{i_p}^{(l)}(t) dt
% \end{aligned}
\label{eq:predict_weights}
\end{equation}
\begin{equation}
% \begin{aligned}
    \Delta \textcolor{NavyBlue}{w_{ji_{pe}}^{(l)}} = -{\rm STDP}(a_{i_p}^{(l)}, e_j^{(l-1)})
    =\eta_{ji_{pe}}\int \left(a_{i_p}^{(l)}(t)\ast \kappa\right)(t)\cdot e_j^{(l-1)}(t)dt
% \end{aligned}
\label{eq:error_weights}
\end{equation}
% \begin{equation}
% \Delta = ?
% \end{equation}
where $\eta_{ij},\eta_{i_pj}$, and $\eta_{ji_{pe}}$ are three different learning rates for these three types of synaptic connections. In the above three equations, all the adjusting rules of a synapse can be described as a STDP or anti-STDP process between a presynaptic current and a postsynaptic error signal, which exploits great biological plausibility. The top-down synaptic weights $\textcolor{Red}{w_{ji_{e}}^{(l)}}$ are set to be equal to the bottom-up forward weights $\textcolor{ForestGreen}{w_{ij}^{(l)}}$ for simplicity. One can also try to initialize the top-down weights $\textcolor{Red}{w_{ji_{e}}^{(l)}}$ as fixed random values following the idea of the feedback alignment (\#cite). 

We interpret each type of synapses' learning rule as following:

In (\ref{eq:forward_weights}), $\textcolor{ForestGreen}{w_{ij}^{(l)}}$ represents the forward weights. It's fixed point $e_i^{(l)}=0$ forms a positive attractor to minimize the error signal. For the output layer, the error signal $e_i^{(l_N)}(t) = a_i^{\rm target}(t) - a_i^{(l_N)}(t)$ also has another meaning, which implies the loss function we used is the Van Rossum distance (\#cite) between a target spike train $s_i^{\rm target}(t)$ and the output spike train $s_i^{(l_N)}$. We denote the loss function by $L = \sum_{i=1}^{N^{(l_N)}}\int E_i(t) dt$, where $N^{(l_N)}$ is the number of pyramidal cells in the output layer $l_N$, and $E_i(t)$ is the loss of the pyramidal cell $i$ at $t$. Specifically, $L$ is given by:
% \vspace{-0.4cm}
\begin{equation}
% \begin{aligned}
    L = \sum_{i=1}^{N^{(l_N)}} \int \frac{1}{2}\left((\epsilon\ast s_i^{\rm target})(t)-(\epsilon\ast s_i^{(l_N)})(t)\right)^2
    =\sum_{i=1}^{N^{(l_N)}} \int \frac{1}{2}\left(a_i^{\rm target}(t) - a_i^{(l_N)}(t)\right)^2
    \label{eq:Loss}
% \end{aligned}
\end{equation}
from which we can get the derivative of $L$ with respect to an output neuron's PSC $a_i^{(l_N)}$ at $t$ equal to our defined error signal $e_i^{(l_N)}(t)$:
\begin{equation}
    \frac{\partial L}{\partial a_i^{(l_N)}(t)} = \frac{\partial E_i(t)}{\partial a_i^{(l_N)}(t)} = \frac{\partial \frac{1}{2}\left(a_i^{\rm target}(t) - a_i^{(l_N)}(t)\right)^2}{\partial a_i^{(l_N)}(t)} = e_i^{(l_N)}(t)
\end{equation}
When training is converged, we expect the error signal $e_i^{(l)}$ of all pyramidal cells $i = 1,\dots, N^{(l)}, l=1,\dots,l_N$ are close to zero, by then $\frac{\partial L}{\partial a_i^{(l_N)}(t)}$ is also close to zero, and an stationary point of $L$ is reached. One can easily integrate other differentiable loss functions into our framework by substituting the error signal $e_i^{(l_N)}$ using the $\frac{\partial L}{\partial a_i^{(l_N)}(t)}$ calculated by their customized loss functions.

In (\ref{eq:predict_weights}), $\textcolor{Orange}{w_{i_pj}^{(l)}}$ stands for the predictive connections. Its fixed point in our learning rule is $e_{i_p}^{(l)}(t) = a_i^{(l)}(t)+a_{i_p}^{(l)}(t) = 0$, which means $s_i^{(l)}(t) = s_{i_p}^{(l)}(t)$ referring to (\ref{eq:negative_psc}). As compared to (\ref{eq:forward_weights}), they do not have a fixed target signal, but need to follow the continuously changing behavior of their corresponding pyramidal cells during training. Empirically, the learning rate $\eta_{i_pj}$ of these predictive connections needs to be larger than the learning rate of the forward connections $\eta_{ij}$ to be able to follow the change of $\eta_{ij}$. 

(\ref{eq:error_weights}) is the only anti-STDP rule as compared to (\ref{eq:forward_weights}) and (\ref{eq:predict_weights}). This is because a SOM cell outputs negative PSC signal ${a}_{i_p}^{(l)}(t) = -(\epsilon \ast {s}_{j_p}^{(l)}) (t)$.
